Space Efficient Approximation to Maximum Matching Size from Uniform Edge Samples

Given a source of iid samples of edges of an input graph $G$ with $n$ vertices and $m$ edges, how many samples does one need to compute a constant factor approximation to the maximum matching size in $G$? Moreover, is it possible to obtain such an estimate in a small amount of space? We show that, on the one hand, this problem cannot be solved using a nontrivially sublinear (in $m$) number of samples: $m^{1-o(1)}$ samples are needed. On the other hand, a surprisingly space efficient algorithm for processing the samples exists: $O(\log^2 n)$ bits of space suffice to compute an estimate. Our main technical tool is a new peeling type algorithm for matching that we simulate using a recursive sampling process that crucially ensures that local neighborhood information from `dense' regions of the graph is provided at appropriately higher sampling rates. We show that a delicate balance between exploration depth and sampling rate allows our simulation to not lose precision over a logarithmic number of levels of recursion and achieve a constant factor approximation. The previous best result on matching size estimation from random samples was a $\log^{O(1)} n$ approximation [Kapralov et al'14]. Our algorithm also yields a constant factor approximate local computation algorithm (LCA) for matching with $O(d\log n)$ exploration starting from any vertex. Previous approaches were based on local simulations of randomized greedy, which take $O(d)$ time {\em in expectation over the starting vertex or edge} (Yoshida et al'09, Onak et al'12), and could not achieve a better than $d^2$ runtime. Interestingly, we also show that unlike our algorithm, the local simulation of randomized greedy that is the basis of the most efficient prior results does take $\wt{\Omega}(d^2)\gg O(d\log n)$ time for a worst case edge even for $d=\exp(\Theta(\sqrt{\log n}))$.

==> 300-overview.tex <==
%!TEX root = ./000-main.tex
\section{Technical Overview}

We now describe the central ideas behind our main result, namely Theorem~\ref{}. As described above, we start with a natural peeling-type algorithm for constructing a constant factor approximation to maximum matching, namely Algorithm~\ref{} below.



==> 400-estimating-matching-size.tex <==
\section{Estimating the Matching Size}
In this section we describe our main result. The section is organized as follows. We first present an algorithm (in \cref{global-algo}) that computes a constant factor approximate fractional maximum matching while having the full access to the graph. Then, in \cref{simul-iid-edge} we provide a simulation of that algorithm on a stream of (iid) edges. The main primitive of our simulation is a procedure (that we also refer by test) that estimates the fractional matching weight incident to a given vertex.
\stodo{We could say that we are combining those estimates, that we obtain independently, to estimate the total matching value.}
Afterward we focus of showing the key properties of the tests that we designed. First in~\cref{sec:sample-complexity} we analyze the sample complexity of our test, then in~\cref{correctness-algo} we show that if we run our test on all the edges, we get a constant approximation guarantee by carefully analyzing the weights that we give to the edges. Afterward in~\cref{sec:all-tests} we show that we do not need to run our test on all the edges and it suffices to run it only till we sampled $O(m)$ iid edges. Putting it all together we get:
\begin{theorem}
For any graph $G=(V,E)$, \cref{alg2} returns a constant approximation guarantee with constant probability, using $\Theta(m)$ sampled edges and memory $O(\log^2 n)$ (stores $O(\log n)$ numbers). 
\end{theorem}



==> 500-coupling.tex <==
\section{Coupling}
Our goal is to bound the total variation distance between the behavior of the algorithm on a stream of edges where each edge is a random sample from the edge set, and the behavior of the algorithm when it is run on a random permutation of the edges. We use the fact that the total variation of two probability distributions $P$ and $Q$ is bounded by $\sqrt{\tfrac{1}{2} \KL{P}{Q}}$, where $\KL{P}{Q}$ is the KL divergence from $Q$ to $P$.

We first consider the following Bernoulli random variables
\[
	X \eqdef \Ber\rb{\rb{1 - \frac{d(u)}{m}}^{m / n}}.
\]
The variable $X$ corresponds to the ``random-edge'' regime when the algorithm performs a $V_1$-test. Here, $X = 0$ if $u$ sees a neighbor among $m/n$ random samples, and $X = 1$ otherwise. In a similar way we define variable $Y$ corresponding to the ``permutation'' regime
\[
	Y \eqdef \Ber\rb{\rb{1 - \frac{\td(u, t)}{(1 - t/m) m}}^{m / n}},
\]
where we use $\td(u, t)$ to denote the degree of $u$ among the edges $e_{t + 1}, \ldots, e_m$ in a given random permutation. We have that
\begin{equation}\label{eq:set-td}
	\frac{\td(u, t)}{1 - t/m} = d(u) \pm O\rb{\sqrt{d(u) \log{1 / \delta}}}
\end{equation}
with probability $1 - \delta$.

We have
\begin{eqnarray*}
	\KL{\Ber(p)}{\Ber(p + \e)} & = & p \log{\frac{p}{p + \e}} + (1 - p) \log{\frac{1 - p}{1 - p - \e}} \\
	& = & \frac{\e^2}{2 p (1 - p)} + O\rb{\frac{\e}{p}}^3 + O\rb{\frac{\e}{1 - p}}^3.
\end{eqnarray*}
\stodo{Perhaps we should expand above why the equality holds.}
Note that the first term in the last equality is dominant -- we have that $\e < 1$; and, $2 p (1 - p) \approx \min\{p, 1 - p\}$ as $2p \ge [1, 2]$ or $2 (1 - p) \ge [1, 2]$.

We now want to bound $\KL{X}{Y}$. In that case, we have
\begin{equation}\label{eq:ee}
	\e = \prob{Y = 1} - \prob{X = 1} = \rb{1 - \frac{d(u) \pm \Delta}{m}}^{m / n} - \rb{1 - \frac{d(u)}{m}}^{m / n},
\end{equation}
where $\Delta \approx \sqrt{d(u) \log{1/\delta}}$ (this is obtained from~\eqref{eq:set-td}).

Now the goal is to bound $\epsilon$. To that end, let us assume that $\frac{d(u)}{m} \leq 1/10$. We show that 
\begin{equation}\label{eq:error}
|\rb{1 - \frac{d(u)}{m}}^{m / n} -\rb{1 - \frac{d(u) \pm \Delta}{m}}^{m / n} |\leq \Theta(|\frac{\Delta}{n}|p).
\end{equation}
where $p =  \rb{1 - \frac{d(u)}{m}}^{m / n}$.
By dividing $\cref{eq:error}$ over by $p$ we need to prove that:
\begin{equation}\label{eq:error}
|1 -\rb{1 - \frac{\Delta}{m(1-\frac{d(u)}{m})}}^{m / n} |\leq \Theta(|\frac{\Delta}{n}|).
\end{equation}
By the assumption that $\frac{d(u)}{m} \leq 1/10$, we get that the LHS is less that
\begin{equation}\label{eq:error}
|\rb{1 - \frac{d(u)}{m}}^{m / n} -\rb{1 - \frac{d(u) \pm \Delta}{m}}^{m / n} |\leq \rb{1-e^{-1.1\frac{\Delta}{n}}} \leq \Theta(|\frac{\Delta}{n}|).
\end{equation}
where the last inequality follows assuming that $\Delta \leq 1000n$.



\begin{lemma}
Assuming that $\epsilon \leq \frac{\Delta}{n}p$, then the $\KL{X}{Y} \leq \frac{1}{n}$
\end{lemma}










==> old-intro.tex <==
A well-studied example occurs in online advertisement, where one needs to learn a graph $G=(A, I, E)$ representing preferences of a set of advertisers for various impressions, and sampling access is a natural assumption \cite{davanur}. 

 \emph{Learning from samples} is a popular regime to studying this question. In this regime, it is assumed that an algorithm performing computation has access to (uniform) samples from the input dataset, and needs to learn a property of the dataset by processing these samples using limited space. 


A well-studied example occurs in online advertisement: a graph $G=(A, I, E)$ representing preferences of a set of advertisers for a set of impressions is implicitly defined, and the task is to allocate i.i.d. samples of impressions arriving online to advertisers so as to maximize the total size of the matching constructed. In this setting one thinks of the `expected' graph $G$ as given, but it is natural for this graph to be estimated through sampling. 



Crouch et al.~\cite{crouch2016stochastic} address this question and study the trade-off between sample and space complexity for several problems, including graph connectivity. Raz~\cite{raz2016fast} studies the problem of parity learning. In this problem, there is an unknown binary string $x \in \{0, 1\}^n$ chosen uniformly at random. The task here is to design an algorithm that receives samples of the form $(a_i, b_i)$, where $a_i \in \{0, 1\}^n$ is a uniformly chosen random vector and $b_i$ is the parity of $a_i \cdot x$, and learns $x$. He shows that any algorithm that uses $o(n^2)$ memory requires an exponential number of samples to solve this task, hence solving a conjecture of Steinhardt et al.~\cite{steinhardt2016memory}. This result is generalized in~\cite{kol2017time, raz2017time}.

Another line of work~\cite{shamir2014fundamental, steinhardt2015minimax} studied learning from samples in the context of statistical learning. \stodo{I am hoping to add something more to this sentence above ...}


\emph{Online stochastic matching} is yet another problem that has received significant attention and that falls under the framework of learning from samples. This problem is motivated by applications in Internet advertising, and is modeled as a bipartite graph $(A, U, E)$ in the following way. We are given a set of advertisers $A$, a set of users $U$ and an edge set $E \subseteq A \times U$. The users arrive online, each user arriving along with its neighbors in $A$. Our goal is to match the users and the advertisers so to maximize the total matching (also called revenue). When $E$ is deterministic, this problem has been studied in several variants~\cite{karp1990optimal,goel2008online,feldman2009online,bahmani2010improved,karande2011online,mahdian2011online,manshadi2012online} depending on knowledge and distribution of $U$. In the \emph{adversarial model}, when there is no prior knowledge of $U$ or $E$, Karp et al.~\cite{karp1990optimal} design a $(1 - 1/e)$-competitive algorithm, and show that this algorithm is optimal. In the \emph{iid model}, where users arrive with repetition according to some known distribution, Goel and Mehta~\cite{goel2008online} prove that the greedy algorithm is $(1 - 1/e)$-competitive. This guarantee was improved by Feldman et al.~\cite{feldman2009online} who design an algorithm for the iid model that is $0.67$-competitive.
\\
Another line of work has considered the variant of online stochastic matching in which $E$ is stochastic. This regime corresponds to the scenario in which after a user and an ad are matched, the user has an option to click on the ad or not. If the user decides to click on the ad, then we consider the match to be successful (and otherwise the match is not successful). If the user clicks on the ad, then the ad is removed from further consideration. On the other hand, if this match is not successful, the ad still can be matched to the users other than $u$ that arrive in the future. To model the behavior of users (whether an ad is clicked or not), it is assumed that to every edge $\{a, u\} \in E$ is assigned probability $p_{a, u}$ that determines the probability that the user $u$ clicks on the ad $a$. The goal of the algorithm is to maximize the number of successfully matched ads from $A$, while not knowing the vector of probabilities $p$. This setting of online stochastic matching was introduced by Mehta and Panigrahi~\cite{mehta2012online}. They study the case when $p$ consists of equal probabilities. They show that if $p_{a, u}$ approaches $0$, then there is a $0.567$-competitive ratio algorithm, which becomes $0.5$-competitive ratio algorithm as $p_{a, u}$ approaches $1$. Mehta et al.~\cite{mehta2015online} study the case of unequal probabilities and show that there is a $0.534$-competitive ratio algorithm when $p_{a, u}$ approaches $0$.
\stodo{We probably should mention some more citations, like~\cite{brubach2016online,assadi2017stochastic,brubach2016new}.}
\fi 

Motivated by the aforementioned scenarios and importance of learning from samples, in this work we consider the problem of estimating the maximum matching size in the setting where edges arrive uniformly at random with repetition. We assume no prior knowledge on the structure of the underlying graph.

==> removed-content.tex <==
\paragraph{General approach and comparison to~\cite{kks2014}} The general idea of our approach is to start by designing a local algorithm for approximating matching size and then convert it into a streaming algorithm using randomness of the stream to perform statistical estimation. In~\cite{kks2014} the authors started with a very simple {\em peeling} algorithm \xxx[MK]{of Parnas and Ron (?)} that gives a factor $O(\log n)$-approximation: the algorithm repeatedly peels off high degree vertices from the graph, finding a large matching in the (somewhat regular) subgraphs that are removed in the process. \cite{kks2014} then shows how to design small space recursive primitives that look at a small fraction of the stream and estimate the execution path of the algorithm. These primitives uses recursion of depth $\Omega(\log n)$, but the fact that \cite{kks2014} achieve a $\log^{O(1)} n$ approximation allows them to reduce the number of recursive calls appropriately. It is crucial for their analysis that the approximation factor is larger than the depth of the recursion. Making this strategy yield a constant factor approximation is challenging exactly because the depth of the recursion is now much larger than the approximation factor. 

The analysis now requires a very delicate approach. \xxx[MK]{Our analysis also yields the first local algorithm with $O(\log d)$ depth and $O(d)$ work.}


\paragraph{Warm Up Algorithm} The main goal of this approach is to design a low memory \emph{peeling algorithm} that iteratively finds the high degree vertices and removes them from the graph. Afterward, to each edge we assign a weight that is a function of the iteration in which this edge was removed from the graph. We show that these weights create a feasible fractional matching and also, by constructing a vertex cover, we prove that our algorithm does not underestimate the size of the matching. More precisely, we will design an algorithm that partitions the vertices into sets $V_T \subseteq V_{T-1} \subseteq \cdots \subseteq V_1$, for $T \in \Theta(\log n)$. The algorithm first finds all the vertices $V_1 \subseteq V$ that have degree less than $n/C$ in the original graph, where $C > 1$ is an absolute constant. We also say that the algorithm \emph{peels} the vertices of degree at least $n / C$.
\stodo{I think that we should split more clearly the full-access algorithm and once we start its simulation. Then when we start describing the simulation, we state the challenges.}
Informally, to decide whether a vertex $v \in V$ should be peeled or not, it suffices to fetch $O(m/n)$ i.i.d. edges from the graph and use them to estimate the degree of $v$ -- if its estimated degree is at least $n / C$, $v$ is removed from the graph and does not appear in $V_1$. Then, the algorithm assigns weight $1/n$ to any edge whose at least one endpoint got peeled. This guarantees that the expected fractional matching assigned to the any such vertex that we remove is $\Theta(1/c)$. The set $V_1$ corresponds to all the vertices that are not peeled in this iteration.

In a similar way, the algorithm finds the vertices having degree less than $n/C^2$ in $V_1$ and removes them from $V_1$ in order to construct $V_2$. To achieve this for a vertex $v \in V_1$ we need $O(Cm/n)$ iid edges, and then based on the number of neighbors that it has in $V_1$ the algorithm estimates its degree in $V_1$. The weight that is assigned to the edges connected to the vertices that got removed in this iteration is $C/n$. The algorithm proceeds in the analogous way to construct all the sets $V_j$.

Prior to this work, the best performance known for a procedure similar to this one was $(\poly \log n)$. In this work we provide a novel analysis that shows that the described algorithm estimates the maximum matching size within a constant factor. A direct implementation of this algorithm requires $\Omega(n)$ memory to store the $V_j$ sets. To avoid this, each time the algorithm needs to learn whether a vertex $v$ belongs to some set $V_j$, it runs the described algorithm above from scratch on $v$. This, in particular, means that the same test could potentially be run on the same vertex multiple times. We use $\vtest{j}{v}$ to refer to the procedure that returns true if $v \in V_j$ and false otherwise. $\vtest{j}{v}$ mimics the approach described above as follows. It queries $\gamma\frac{c^{j-1}m}{n}$ i.i.d. edges and for any neighbor $u$ of $v$ among the sampled edges it runs $\vtest{j - 1}{u}$. If for any $u$ the outcome of $\vtest{j - 1}{u}$ is true, the algorithm returns false for $\vtest{j}{v}$. Intuitively, if $\vtest{j - 1}{u}$ returns true it means that $v$ has degree at least $\gamma\frac{n}{c^{j-1}}$ so it should be removed from $V_j$. Here is this test in more details\todo{we want this?}. Unfortunately, the number of samples that this test uses - even if we run them carefully - for even one vertex can potentially be $\omega(m \log n)$. More precisely, $\vtest{j}{v}$ might use $\omega(c^jm/n \log n)$ i.i.d. edges, therefore we need to design a more efficient test.

\paragraph{Early Stopping Tests} One of the main challenges we face in this work is to estimate the maximum matching size by using only $O(m)$ iid edge-samples. To achieve that, on a high-level, we track (an approximate) number of samples used while testing a given vertex and if we realize that there are ''too many`` of them used so far, we simply terminate the execution. We call this the \emph{early stopping rule}. This idea is implemented in the following way. For each instance of $\vtest{j}{v}$, the algorithm maintains variable $S$. The role of $S$ is to count the number of samples that are used while testing $\vtest{j}{v}$. We note that $S$ corresponds to the number of samples properly scaled, as made precise next. Initially, $S = 0$. As discussed above, the algorithm samples $O(\gamma \frac{c^{j-1}m}{n})$ i.i.d.~edges and for each neighbor $u$ of $v$ runs $\vtest{i}{u}$ starting from $i=0$. If $u$ passes this test, $S$ is incremented by $c^{i-j}$. After each increment, the algorithm tests whether $S \geq \delta$, where $\delta$ is a constant that we fix later. If $S \ge \delta$, the algorithm returns \false for $\vtest{j}{v}$. Here, returning \false corresponds to terminating the execution of that test early. Also, the value of $S$ is incremented non-uniformly, and depends on which test is directly invoked by $\vtest{j}{v}$. Intuitively, when $\vtest{j}{v}$ invokes $\vtest{i}{v}$ for small $i$, such $\vtest{i}{v}$ require a small number of iid samples for its execution. Hence, the algorithm increments $S$ by little in that case. If, on the other hand, $i$ is very close to $j$, $\vtest{i}{v}$ requires many samples and hence the algorithm increments $S$ by a lot more than in the previous case.

We now argue why the early stopping rule does not affect the approximation guarantee. Intuitively, the new test also estimates the amount of fractional matching that the removed edges neighboring a vertex has and stops adding more weight as soon as the summation of these weights are big. Opposing to the previous page which almost ignored the weight of the previously added edges and simply peeled a vertex when the it was in a layer that the summation of the weights in this particular layer was high. This gives us two main advantages
\begin{enumerate}
\item We peel off vertices that their degree is close to the threshold earlier, which reduces the number of sampled edges significantly.
\item Gives us a better understanding why the summation of the weights assigned to a vertex is not too high.
\end{enumerate}
We explain this approach in more details in the next section. We also highlight some of the key ideas that we use in the analysis in \cref{correctness-algo}.

\paragraph{Lower-Bound on the Number of Sampled Edges} In this work, we show that to achieve a constant approximation guarantee, it is necessary to sample $\Omega(m)$ iid edges. More precisely, for any fixed constant $c$, we first present two sparse graphs $G_1, G_2$ with $n$ vertices and $O(n)$ edges, such that their matching size differs by a factor $c$. Moreover, we show that sampling $O(n^{1-\epsilon})$ edges is not sufficient to differentiate these to graphs. Then we add two big cliques of size $n/c$ two $G_1$ and $G_2$ to construct to new graphs $G'_1$ and $G'_2$. Intuitively, of any $n/c$ edges that one samples from $G'_1$ and $G'_2$, only one edge is sampled from the sparse part. This results to losing an extra factor $n/c$ in the number of the edges that needed to be sampled to differentiate between these to graphs. Therefore, we get that one needs at least $\omega(n^{2-\epsilon})$ iid edges in order to find a constant approximation guarantee for the size of the matching. Notice that, the in inapproximibility that we show, holds for any memory. Basically, regardless of the memory that the algorithm uses, it cannot distinguish $G'_1, G'_2$ without desired number of sampled edges. We present the details of our structure in \cref{sec:lower-bound}.


==> useful-stuff-forests.tex <==
    We will write the number of embeddings of $F$ into $G$ (resp. $H$) in terms of the number of embeddings of $F_1$,  $F_2$ into $G$ (resp. $H$), as well as embeddings of natural derived forests. 
    
    Indeed, every pair of embeddings $(\Psi_1, \Psi_2)$, where $\Psi_i: V_{F_i}\hookrightarrow V_G, i\in \{1, 2\},$ naturally defines a mapping $\Phi:V_F\to V_G$. However, this mapping is not necessarily injective. We quantify this now using the notion of a {\em clashing pair} of embeddings $(\Psi_1, \Psi_2)$. 
    
    \begin{definition}
    Let a clashing function between $F_1$ and $F_2$ be a mapping $\xi:V_{F_1}\to V_{F_2}\cup\{\star\}$, such that $\not\exists u,w\in V_{F_1}:\xi(u)=\xi(w)\not=\star$. That is $\xi$ is almost but not quite an injection, two vertices may both be mapped to $\star$. If an pair of embeddings of $F_1$ and $F_2$ into $G_i$ clash via $\xi$ it means that the images of $u$ and $\xi(u)$ coincide in $V_i$. If for a vertex of $F_1$ $\xi(u)=\star$, it means that the vertex clashes with nothing and does not violate the injectivity requirement.
    
    Let the set of all possible clashing functions be
    $$\Xi=\left\{\xi:V_{F_1}\to V_{F_2}\cup\{\star\}\middle|\not\exists u,w\in V_{F_1}:\xi(u)=\xi(w)\not=\star\ \wedge\ \exists u\in V_{F_1}:\xi(u)\not=\star\right\}$$
    That is we exclude the constant $\star$ function, as it would represent no clashing between the two embeddings.
    \end{definition}
    
    For any clashing function $\xi\in\Xi$ we need to quantify the pairs of embeddings $(\Phi_1,\Phi_2)$ that clash via $\xi$. Finding a pair of $\xi$-clashing embeddings of $F_1$ and $F_2$ like this is equivalent to finding a single embedding of a slightly modified graph: one that is similar to $F$ but the clashing vertices have been merged. We make this more formal.
    
    \begin{definition}
    Let $\xi\in\Xi$. Define the graph $F_1\stackrel{\xi}{+}F_2$ as follows. Its vertex set is $\xi^{-1}(\star)\cup V_{F_2}$. Two of its vertices, $u$ and $w$, are connected by an edge under the following circumstances:
    \begin{itemize}
        \item Both $u$ and $w$ are in $V_{F_1}$ and they are connected in $E_{F_1}$.
        \item Both $u$ and $w$ are in $V_{F_2}$ and they are connected in $E_{F_2}$.
        \item $u$ and $w$ come from different vertex sets, say $u\in V_{F_1}$ and $w\in V_{F_2}$, and there exists a preimage of $w$ in $\xi$ such that it is connected to $u$ in $E_{F_1}$.
    \end{itemize}
    \end{definition}
    
   \begin{observation}{\label{gamma}}
   The number of embedding-pairs $(\Phi_1,\Phi_2)$ that clash exactly via $\xi$ is equal to the number of embeddings of $F_1\stackrel{\xi}+F_2$ into $G_i$, ie. $\widetilde\Gamma_i^{F_1\stackrel{\xi}+F_2}$. Note that $F_1\stackrel{\xi}+F_2$ may not be a forest, in which case this quantity is $0$.
   \end{observation}
   
   \begin{observation}{\label{comp-red}}
   For any $\xi\in\Xi$, $F_1\stackrel{\xi}+F_2$ is a graph with fewer connected components than $Q$.
   \end{observation}


    

    
    
   
   We are now ready to finish the proof; we will count the number of embeddings of $F$ by independently counting the number of emebeddings of $F_1$ and $F_2$ and subsequently subtracting invalid (clashing) pairs. For easier notation, let $\widetilde\Gamma_i^{F_1\stackrel{\xi}+F_2}=\widetilde\Gamma_i^\xi$.
   \begin{align*}
       \widetilde\Gamma_1^F&=\widetilde\Gamma_1^{F_1}\cdot\widetilde\Gamma_1^{F_2}-\enum{(\Phi_1,\Phi_2)}{\Phi_1\text{ and }\Phi_2\text{ clash}}\\
       &=\widetilde\Gamma_1^{F_1}\cdot\widetilde\Gamma_1^{F_2}-\sum_{\xi\in\Xi}\enum{(\Phi_1,\Phi_2)}{\Phi\text{ and }\Phi_2\text{ clash via }\xi}\\
       &=\widetilde\Gamma_1^{F_1}\cdot\widetilde\Gamma_1^{F_2}-\sum_{\xi\in\Xi}\widetilde\Gamma_1^\xi\\
       &=\widetilde\Gamma_2^{F_1}\cdot\widetilde\Gamma_2^{F_2}-\sum_{\xi\in\Xi}\widetilde\Gamma_2^\xi\\
       &=\widetilde\Gamma_2^F
   \end{align*}
    Here we used observation \ref{comp-red} to allow us to use the inductive hypothesis on $\widetilde\Gamma_1^\xi$ in cases where $F_1\stackrel{\xi}+F_2$ is a forest. In cases where it is not, both $\widetilde\Gamma_1^\xi$ and $\widetilde\Gamma_2^\xi$ are $0$.


==> useful-stuff.tex <==
==========
We first prove 
\begin{lemma}
For every integers $c\geq 1$, $k\geq 2$, $i=1,\ldots, c$ the size of the special set of vertices in $\bar G^{(j)}_i$ is the same as in $\bar H^{(j)}_i$, and the degrees of the special vertices in $\bar G^{(j)}_i$ and $\bar H^{(j)}_i$ are equal.
\end{lemma}

\paragraph{Base case: $j=2$.} Since the minimum degree in $G^{(1)}$ equals $l=1$ the maximum degree equals $h=c+1$,  the graph $\bar G^{(2)}_i, i=1,\ldots, c$ contains $h-l=c$  special vertices. The degrees of the special vertices are all $(c+1)c$, as they connect to all low degree nodes in $G^{(1)}$ (i.e., the $c(c+1)$ endpoints of the $c(c+1)/2$ isolated edges). Since the minimum degree in $H^{(1)}$ equals $l=1$ the maximum degree equals $h=c+1$,  the graph $\bar H^{(2)}_i, i=1,\ldots, c$ contains $h-l=c$  special vertices. The degrees of the special vertices are all $(c+1)c$, as they connect to all low degree nodes in $G^{(1)}$ (i.e., the $c(c+1)$ petals of the $c+1$ stars with $c$ petal each). This establishes the base case.


\paragraph{Inductive step: $j-1\to j$.} Now define $\Phi^{(j)}$ by induction on $j$ as follows. Recalling that $G^{(j)}$ is a disjoint union of $c$ copies of the degree paddings $\bar G^{(j-1)}$ of $G^{(j-1)}$, and $H^{(j)}$ is a disjoint union of $c$ copies of the degree padding $\bar H^{(j-1)}$ of $H^{(j-1)}$, we note that it suffices to define a bijection $\bar \Phi^{(j-1)}$ from $\bar H^{(j-1)}$ to $\bar G^{(j-1)}$ from a bijection $\Phi^{(j-1)}$ from $H^{(j-1)}$ to $G^{(j-1)}$, which we assume has been constructed by the inductive hypothesis. By part {\bf (B)} of the inductive hypothesis we have that the size of the special set of vertices in $\bar G^{(j-1)}_i$ for every $i=1,\ldots, c$ is the same as the size of the special set of vertices in $\bar H^{(j-1)}_i, i=1,\ldots, c$. We can thus define the bijection $\Phi^{(j)}$ by mapping the special set $A_i$ of vertices in $\bar H^{(j-1)}_i$ bijectively (in an arbitrary way otherwise) to the special set $B_i$ of vertices in $\bar G^{(j-1)}_i$, and mapping the complement of the special set of vertices in $\bar H^{(j-1)}$ to the complement of the special set in $\bar G^{(j-1)}_i$ using $\Phi^{(j-1)}$.
========


We prove 
\begin{lemma}
For every integers $c\geq 1$, $k\geq 1$, if $\wt{G}:=G^{(k)}$ and $\wt{H}:=H^{(k)}$ are as defined in~\eqref{}, then there exists a bijection $\Phi:V_{\wt{H}}\to V_{\wt{G}}$ such that for every $v\in V_{\wt{G}}$ one has $d_j^{\wt{H}}(v)=d_j^{\wt{G}}(\Phi(v))$.
\end{lemma}
\begin{proof}
We define a bijection $\Phi^{(j)}$ by induction on $j=1,\ldots, k$, and then let $\Phi:=\Phi^{(k)}$.  We will prove the following claims by induction on $j$:
\begin{description}
\item[(A)] There exists a bijection $\Phi^{(j)}$ from $H^{(j)}$ to $G^{(j)}$ such that for every $v\in H^{(j)}$ one has $d_j^{H^{(j)}}(v)=d_j^{G^{(j)}}(\Phi^{(j)}(v))$.
\item[(B)] For every $i=1,\ldots, c$, the size of the special set of vertices in $\bar G^{(j)}_i$ is the same as in $\bar H^{(j)}_i$, and the degrees of the special vertices in $\bar G^{(j)}_i$ and $\bar H^{(j)}_i$ are equal.
\end{description}

\paragraph{Base case: $j=1$.} We start by defining the bijection $\Phi^{(1)}$ from $H^{(1)}$ to $G^{(1)}$ that maps vertices of $H^{(1)}$ to vertices of the same degree in $G^{(1)}$ bijectively (we verify below that this is well-defined).


\paragraph{Inductive step: $j-1\to j$.} Now define $\Phi^{(j)}$ by induction on $j$ as follows. Recalling that $G^{(j)}$ is a disjoint union of $c$ copies of the degree paddings $\bar G^{(j-1)}$ of $G^{(j-1)}$, and $H^{(j)}$ is a disjoint union of $c$ copies of the degree padding $\bar H^{(j-1)}$ of $H^{(j-1)}$, we note that it suffices to define a bijection $\bar \Phi^{(j-1)}$ from $\bar H^{(j-1)}$ to $\bar G^{(j-1)}$ from a bijection $\Phi^{(j-1)}$ from $H^{(j-1)}$ to $G^{(j-1)}$, which we assume has been constructed by the inductive hypothesis. By part {\bf (B)} of the inductive hypothesis we have that the size of the special set of vertices in $\bar G^{(j-1)}_i$ for every $i=1,\ldots, c$ is the same as the size of the special set of vertices in $\bar H^{(j-1)}_i, i=1,\ldots, c$. We can thus define the bijection $\Phi^{(j)}$ by mapping the special set $A_i$ of vertices in $\bar H^{(j-1)}_i$ bijectively (in an arbitrary way otherwise) to the special set $B_i$ of vertices in $\bar G^{(j-1)}_i$, and mapping the complement of the special set of vertices in $\bar H^{(j-1)}$ to the complement of the special set in $\bar G^{(j-1)}_i$ using $\Phi^{(j-1)}$.

%        \begin{claim}{\label{nested-induction}}
%            For any $v\in V_1^{(j-1)}\cup W_1$ and $v'\in V_2^{(j-1)\cup W_2}$ such that $\widetilde\Phi^{(j)}(v)=v'$, $d_j^{\widetilde G_1^{(j)}}(v)=d_j^{\widetilde G_2^{(j)}}(v')$.
%            \jakab{this looks terrible. so much notation. also it's nested induction which is not very nice.}
%        \end{claim}


            For easier notation, for rest of the proof of claim \ref{nested-induction} let $d_\iota(v)$ denote either $d_\iota^{G_1^{(j-1)}}(v)$ or $d_\iota^{G_2^{(j-1)}}(v)$ depending on which vertex-set $v$ actually resides in. Also, let $\tilde d_\iota(v)$ denote $d_\iota^{\widetilde G_1^{(j)}}(v)$ or $d_\iota^{\widetilde G_2^{(j)}}(v)$. Similarly, let $N(v)$ and $\widetilde N(v)$ denote the neighborhood of $v$ in $G_i^{(j-1)}$ and $\widetilde G_i^{(j)}$ respectively, for the appropriate choice of $i$ in each case.
            With this notation in place, we prove the following two claims simultaneously by induction:
            \begin{enumerate}
                \item For any $u\in V_1^{(j-1)}$ and $u'\in V_2^{(j-1)}$ (not necessarily connected by any bijection) if $d_{\iota-1}(u)=d_{\iota-1}(u')$ then $\tilde d_\iota(u)=\tilde d_\iota(u')$. (For the purposes of this statement Let $d_0^G(v)=\emptyset$ always.)
                \item For any $w\in W_1$ and $w'\in W_2$ $\tilde d_\iota(w)=\tilde d_\iota(w')$.
            \end{enumerate}
            \textbf{Base case($\iota=1$):}
            \begin{enumerate}
                \item By construction of $\widetilde G_i^{(j)}$, all vertices in either $V_1^{(j-1)}$ or $V_2^{(j-1)}$ have degree exactly $d_H^{(j-1)}$, so the claim that their $1$-level degrees match is true.
                \item By construction of $\widetilde G_i^{(j)}$, all vertices in either $W_1$ or $W_2$ have degree exactly $N_L^{(j-1)}$, so the claim that their $1$-level degrees match is true.
            \end{enumerate}
            \textbf{Inductive step ($\iota-1\to\iota$):}
                
                \begin{enumerate}
                
                \item Suppose we have two vertices $u$ and $u'$ satisfying the condition from claim (a), ie. $d_{\iota-1}(u)=d_{\iota-1}(u')$. Then, by definition
                $$\biguplus_{\omega\in N(u)}d_{\iota-2}(\omega)=\biguplus_{\omega'\in N(u')}d_{\iota-2}(\omega')$$
                This means that there exists a bijection between the ($G_i^{(j-1)}$-)neighborhoods of $u$ and $u'$, $\Phi_u^*:N(u)\to N(u')$ that preserves $\iota-2$-level degrees. For any $\omega\in N(u)$ and $\omega'\in N(u')$ such that $\Phi_u^*(\omega)=\omega'$, by claim (a) of the inductive hypothesis it is also true that $\tilde d_{\iota-1}(\omega)=\tilde d_{\iota-1}(\omega')$. Therefore:
                $$\biguplus_{\omega\in N(u)}\tilde d_{\iota-1}(\omega)=\biguplus_{\omega'\in N(u')}\tilde d_{\iota-1}(\omega')$$
                Here we're almost done; in order to prove the inductive step for claim (a), we must show that
                $$\biguplus_{\omega\in\widetilde N(u)}\tilde d_{\iota-1}(\omega)=\biguplus_{\omega'\in\widetilde N(u')}\tilde d_{\iota-1}(\omega')$$
                Notice that $N$ is replaced by $\widetilde N$ in both places compared to the previous equality. That is, in order to finish we need to take the multiset-union over the neighborhood in $\widetilde G_i^{(j)}$ not in $G_i^{(j-1)}$.
                
                \textbf{Case 1:} Suppose $u$ is in $V_{1,H}^{(j-1)}$. It follows that $u'$ is also in $V_{2,H}^{(j-1)}$. Then we are already done, since $u$ is not connected to $W_1$ and its neighborhoods in $G_1^{(j-1)}$ and $\widetilde G_1^{(j)}$ are identical. Similarly for $u'$.
                
                \textbf{Case 2:} Suppose now that $u$ is in $V_{1,L}^{(j-1)}$. It follows that $u'$ is also in $V_{2,L}^{(j-1)}$. Then $\widetilde N(u)\backslash N(u)=W_1$. Similarly $\widetilde N(u')\backslash N(u')=W_2$. We know that $|W_1|=|W_2|$ and by claim (b) of the inductive hypothesis any pair of vertices in $W_1$ and $W_2$ respectively has identical $\tilde d_{\iota-1}$-degree. Therefore, extending the multiset-union from $N(u)$ and $N(u')$ to $\widetilde N(u)$ and $\widetilde N(u')$ will not disrupt the equality.
                
                In both cases we have showed that $\tilde d_\iota(u)=\tilde d_\iota(u')$ as claimed.
                \item Suppose now that we have two vertices $w\in W_1$ and $w'\in W_2$. In this case $\widetilde N(w)=V_{1,L}^{(j-1)}$ and $\widetilde N(w)=V_{2,L}^{(j-1)}$ so we must prove that
                $$\biguplus_{\omega\in V_{1,L}^{(j-1)}}\tilde d_{\iota-1}(\omega)=\biguplus_{\omega'\in V_{2,L}^{(j-1)}}\tilde d_{\iota-1}(\omega')$$
                or equivalently that there exists a bijection between $V_{1,L}^{(j-1)}$ and $V_{2,L}^{(j-1)}$ that preserves $\tilde d_{\iota-1}$-degree.
                
                We know from claim (d) of the {\it outer} inductive hypothesis that a bijection $\Phi^{(j-1)}$ exists that preserves the $d_{j-1}$-degree between $V_1^{(j-1)}$ and $V_2^{(j-1)}$. Clearly, $\Phi^{(j-1)}$ must map $V_{1,L}^{(j-1)}$ to $V_{2,L}^{(j-1)}$. Since $\Phi^{(j-1)}|_{V_{1,L}^{(j-1)}}$ preserves $d_{j-1}$ degree it also preserves $d_{\iota-2}$-degree and by claim (a) of the {\it inner} inductive hypothesis it also preserves $\tilde d_{\iota-1}$-degree. Thus it is an appropriate bijection and claim (b) holds.
                \end{enumerate}
                
            To conclude the proof of claim \ref{nested-induction} consider again a vertex $v\in V_1^{(j-1)}\cup W_1$ to which $\widetilde\Phi^{(j)}$ can be applied. If $V$ is in $V_1^{(j-1)}$ then the claim holds by (a); if it is in $W_1$ then the claim holds by (b).
     \end{proof}






















......................................................................................................................



















In the following section we will prove that our algorithm is nearly optimal with respect to sample complexity, even disregarding the constraint on space. That is to say, with polynomially fewer than $m$ samples it is impossible to approximate the matching number of the graph to within a constant factor. We state this more formally:

\begin{theorem}\label{lower-mainmain}
For any $\epsilon>0$ and $C>0$ there exists a pair of graphs, $\widehat G_1$ and $\widehat G_2$, such that their matching number differ by a factor of at least $C$. However, when both are edge-sampled at rate $n^{2-\epsilon}$, the two outcomes are within inverse polynomial total variation distance of each other, modulo isomorphism.
\end{theorem}

In our construction our main tool will be a pair of constant sized graphs that are indistinguishable if only some given constant number of edges are sampled from either. Formally:

\begin{theorem}{\label{lower-main}}
For every $\lambda>1$ there exist graphs $G$ and $H$ such that $\mm G\ge\lambda\cdot\mm H$, but for every graph $K$ with at most $k$ edges, the number of subgraphs of $G$ and $H$ isomorphic to $K$ are equal.
\end{theorem}

\begin{construction}{\label{con-main}}

Construction of $\wh G_1$ and $\wh G_2$ for \cref{lower-mainmain}. Invoke \cref{lower-main} with parameters $\lambda=2C$ and $k=2/\epsilon$ to get the pair of constant-sized graphs $G_1$ and $G_2$. Let the number of vertices of $G_1$ and $G_2$ be $\mathcal N_1$ and $\mathcal N_2$ respectively; let $\mathcal N=\max\left(\mathcal N_1,\mathcal N_2\right)$. (In reality our construction guarantees $\mathcal N_1=\mathcal N_2$ but this is not important here.) Let the matching number of $G_2$ be $\mathcal M$. This guarantees that the matching number of $G_1$ is at least $\lambda\mathcal M=2C\mathcal M$.

Our construction is the following. For $i\in\{1,2\}$ we take $\frac n{2\mathcal N}$ disjoint copies of $G_i$, then add a clique of size $\mu n$ where $\mu=\frac{\mathcal M}{\mathcal N}$. Let the resulting graph be $\wh G_i$.

\end{construction}

\begin{proof}

Proof of \cref{lower-mainmain}, we are working with construction \ref{con-main}. First note that matching number of $\wh G_1$ is at least $\frac n{2\mathcal N}$ times that of $G_1$, so at least $\frac{C\mathcal Mn}{\mathcal N}$. On the other hand, in $\wh G_2$, $\frac{\mathcal Mn}{2\mathcal N}$ matching comes from the copies of $G_2$ and $\frac{\mu n}2=\frac{\mathcal Mn}{2\mathcal N}$ matching comes from the clique: a total of $\frac{\mathcal Mn}{2\mathcal N}$.

Consider the graph of $n^{2-\epsilon}$ iid sampled edges of $\wh G_1$ and $\wh G_2$ respectively. We wish to bound the total variation distance of the two outcomes. Since both graphs have at least $\mu^2n^2/3$ edges this means that the expected number of times any single edge occurs is at most $\frac{3n^{-\epsilon}}{\mu^2}$, and the probability that it occurs is between $0$ and $\frac{3n^{-\epsilon}}{\mu^2}$ by Markov's inequality. Consider a single instance of $G_i$, call it $G_i^*$. $G_i^*$ has at most $\mathcal N^2$ edges, so the probability that more than $k$ of them will occur in the stream is at most
$$\binom{\mathcal N^2}{k+1}\cdot\left(\frac{3n^{-\epsilon}}{\mu^2}\right)^{k+1}\le\binom{\mathcal N^2}{k+1}\cdot\left(\frac{3}{\mu^2}\right)^{k+1}\cdot n^{-2}$$
by union bound. Again by union bound, the probability that any single instance of $G_i$ has more than $k$ of its edges occur in the stream is at most
$$\binom{\mathcal N^2}{k+1}\cdot\left(\frac{3}{\mu^2}\right)^{k+1}\cdot\frac1{2\mathcal N}\cdot n^{-1}=\mathcal O_{C,\epsilon}(n^{-1})$$
We will show that the distribution of sampled graphs $\wh G_1$ and $\wh G_2$ are identical, modulo isomorphism, conditioned on the event that no single instance of $G_1$ ($G_2$ respectively) has more than $k$ of its edges occur in the stream.

Clearly, the cliques are identical in the two graphs and so are the distributions of their subsampled versions. Consider again a pair of copies of $G_1$ and $G_2$, $G_1^*$ and $G_2^*$. We must show that their subsampled versions are identical in distribution give that neither has more than $k$ edges sampled. Note that $G_1^*$ and $G_2^*$ have the same number of edges (indeed, just apply the guarantee of \cref{lower-main} with $H$ being a single edge), call this number $\mathcal E$. It follows that for any specific number $l\le k$, the probability of exactly $l$ edges of $G_1^*$ occuring is exactly the same as the probability of exactly $l$ edges of $G_2^*$ occuring. Furthermore, consider any fixed $l$, and subgraph $H$ of $l$ edges. The probability that the sampled version $G_i^*$ is exactly isomorphic to $H$, given that $l$ edges are sampled is
$$\frac{\enum{K\subseteq G_i^*}{K\cong H}}{\binom{\mathcal E}l}$$
which is the same for both values of $i$ ($1$ and $2$) by the guarantee of \cref{lower-main}. ($K\subseteq G$ denotes that $K$ is a subgraph of $G$.)

Thus we cannot distinguish between $\wh G_1$ and $\wh G_2$ with probability more than $\frac12+\mathcal O_{C,\epsilon}(n^{-1})$.



\end{proof}
